Accounting for data heterogeneity in integrative analysis and prediction methods: An application to Chronic Obstructive Pulmonary Disease

Epidemiologic and genetic studies in chronic obstructive pulmonary disease (COPD) and many complex diseases suggest subgroup disparities (e.g., by sex). We consider this problem from the standpoint of integrative analysis where we combine information from different views (e.g., genomics, proteomics, clinical data). Existing integrative analysis methods ignore the heterogeneity in subgroups, and stacking the views and accounting for subgroup heterogeneity does not model the association among the views. To address analytical challenges in the problem of our interest, we propose a statistical approach for joint association and prediction that leverages the strengths in each view to identify molecular signatures that are shared by and specific to males and females and that contribute to the variation in COPD, measured by airway wall thickness. HIP (Heterogeneity in Integration and Prediction) accounts for subgroup heterogeneity, allows for sparsity in variable selection, is applicable to multi-class and to univariate or multivariate continuous outcomes, and incorporates covariate adjustment. We develop efficient algorithms in PyTorch. Our COPD findings have identified several proteins, genes, and pathways that are common and specific to males and females, some of which have been implicated in COPD, while others could lead to new insights into sex differences in COPD mechanisms.

==> Tables/Tab_Kselect_Full.tex <==
%% Last updated on 17MAY2023

%% Full Overlap Table
\begin{table}[htbp]
\caption{K Selection Simulation Results, Full Overlap Scenario. 
We calculated eigenvalues of the correlation matrix of either the concatenated $\bm X$ matrix or each $X^{d,s}$ matrix separately. We look at the percent of additional variation that is explained from one component to the next adding components until the additional proportion of variance explained is less than the given threshold. In the \textit{simple} approach, we  look at the change in percent variation until it drops below the given threshold. The 'K Selected' columns are the proportion of times that value of K was selected for the given data approach, setting, and threshold. Results are based on 20 simulated data sets. Variable dimensions are P1 = [300, 350], P2 = [1000, 1500], and P3 = [2000, 3000]. Of these variables, the same 50 variables are important to each subgroup, and there are no variables unique to each subgroup.}\label{tab_Kselect_Full}%
\begin{tabular}{@{}cccccccccccc@{}}
\toprule
\multicolumn{3}{c}{ } & \multicolumn{9}{c}{K Selected} \\
\cmidrule(l{3pt}r{3pt}){4-12}
Data & Setting & Threshold & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10\\
\midrule
 &  & 0.10 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00\\

 &  & 0.15 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\

 &  & 0.20 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\

 & \multirow[t]{-4}{*}{\centering\arraybackslash Full P1} & 0.25 & 0.00 & 0.20 & 0.80 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\
\cmidrule{2-12}
 &  & 0.10 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00\\

 &  & 0.15 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00\\

 &  & 0.20 & 0.00 & 0.00 & 0.90 & 0.10 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\

 & \multirow[t]{-4}{*}{\centering\arraybackslash Full P2} & 0.25 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\
\cmidrule{2-12}
 &  & 0.10 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00\\

 &  & 0.15 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00\\

 &  & 0.20 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\

\multirow[t]{-12}{*}{\centering\arraybackslash Concatenated} & \multirow[t]{-4}{*}{\centering\arraybackslash Full P3} & 0.25 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\
\cmidrule{1-12}
 &  & 0.10 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00\\

 &  & 0.15 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\

 &  & 0.20 & 0.00 & 0.80 & 0.20 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\

 & \multirow[t]{-4}{*}{\centering\arraybackslash Full P1} & 0.25 & 0.15 & 0.85 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\
\cmidrule{2-12}
 &  & 0.10 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.20 & 0.80\\

 &  & 0.15 & 0.00 & 0.00 & 0.00 & 0.00 & 0.70 & 0.30 & 0.00 & 0.00 & 0.00\\

 &  & 0.20 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\

 & \multirow[t]{-4}{*}{\centering\arraybackslash Full P2} & 0.25 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\
\cmidrule{2-12}
 &  & 0.10 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00\\

 &  & 0.15 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00\\

 &  & 0.20 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\

\multirow[t]{-12}{*}{\centering\arraybackslash Separate} & \multirow[t]{-4}{*}{\centering\arraybackslash Full P3} & 0.25 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\
\bottomrule
\end{tabular}
\end{table}




==> Tables/Tab_Kselect_Partial.tex <==
%% Last updated 17MAY2023

%% Partial Overlap Table
\begin{table}[htbp]
\caption{K Selection Simulation Results, Partial Overlap Scenario. 
We calculated eigenvalues of the correlation matrix of either the concatenated $\bm X$ matrix or each $X^{d,s}$ matrix separately. We look at the percent of additional variation that is explained from one component to the next adding components until the additional proportion of variance explained is less than the given threshold. In the \textit{simple} approach, we  look at the change in percent variation until it drops below the given threshold. The 'K Selected' columns are the proportion of times that value of K was selected for the given data approach, setting, and threshold. Results are based on 20 simulated data sets. Variable dimensions are P1 = [300, 350], P2 = [1000, 1500], and P3 = [2000, 3000]. Of these variables, 25 are important to each subgroup, and there are 25 variables that are unique to each subgroup.}\label{tab_Kselect_Partial}%
\begin{tabular}{@{}cccccccccccc@{}}
\toprule
\multicolumn{3}{c}{ } & \multicolumn{9}{c}{K Selected} \\
\cmidrule(l{3pt}r{3pt}){4-12}
Data & Setting & Threshold & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10\\
\midrule
 &  & 0.10 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00\\

 &  & 0.15 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\

 &  & 0.20 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\

 & \multirow[t]{-4}{*}{\centering\arraybackslash Partial P1} & 0.25 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\
\cmidrule{2-12}
 &  & 0.10 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00\\

 &  & 0.15 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00\\

 &  & 0.20 & 0.00 & 0.00 & 0.75 & 0.25 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\

 & \multirow[t]{-4}{*}{\centering\arraybackslash Partial P2} & 0.25 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\
\cmidrule{2-12}
 &  & 0.10 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00\\

 &  & 0.15 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00\\

 &  & 0.20 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\

\multirow[t]{-12}{*}{\centering\arraybackslash Concatenated} & \multirow[t]{-4}{*}{\centering\arraybackslash Partial P3} & 0.25 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\
\cmidrule{1-12}
 &  & 0.10 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00\\

 &  & 0.15 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\

 &  & 0.20 & 0.00 & 0.80 & 0.20 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\

 & \multirow[t]{-4}{*}{\centering\arraybackslash Partial P1} & 0.25 & 0.10 & 0.90 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\
\cmidrule{2-12}
 &  & 0.10 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.10 & 0.90\\

 &  & 0.15 & 0.00 & 0.00 & 0.00 & 0.00 & 0.75 & 0.25 & 0.00 & 0.00 & 0.00\\

 &  & 0.20 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\

 & \multirow[t]{-4}{*}{\centering\arraybackslash Partial P2} & 0.25 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\
\cmidrule{2-12}
 &  & 0.10 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00\\

 &  & 0.15 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00\\

 &  & 0.20 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\

\multirow[t]{-12}{*}{\centering\arraybackslash Separate} & \multirow[t]{-4}{*}{\centering\arraybackslash Partial P3} & 0.25 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\
\bottomrule
\end{tabular}
\end{table}


==> Tables/Tab_RDA_dem.tex <==
%  Last updated 02MAY2023

% Manual changes 01JUN2023
%   Airway WALL Thickness label
%   Remove SBP and DBP
%   Remove ", Thirona" from emphysema
%   Changed "Caucasian" to "Non-Hispanic White"


% Removed from caption since no longer include BP in table: Systolic and diastolic blood pressure values are an average of 3 measurements taken at the Year 5 visit.

%Systolic Blood Pressure (avg) & 130.07 (16.75) & 129.25 (16.84) & 0.367\\
%Diastolic Blood Pressure (avg) & 76.21 (10.19) & 74.20 (10.39) & $<$0.001\\

\begin{table}[htbp]
\caption{COPDGene Participant Characteristics. The measurements presented were collected at the Year 5 study visit to align with the collection of proteomic and genomic data collection. }\label{tab_RDA_dem}%
\begin{tabular*}{\textwidth}{@{\extracolsep\fill}lcccccc}
\toprule
\multicolumn{1}{c}{Variable} & \multicolumn{1}{c}{Males} & \multicolumn{1}{c}{Females} & \multicolumn{1}{c}{P-value} \\
  & N = 782 & N = 594 &  \\
\midrule
Age & 68.28 (8.35) & 68.03 (8.36) & 0.581\\
BMI & 28.03 (5.62) & 27.69 (6.59) & 0.317\\
FEV1 \% Predicted & 61.94 (22.97) & 62.91 (22.59) & 0.431\\
BODE Index & 2.45 (2.45) & 2.63 (2.38) & 0.176\\
\% Emphysema & 11.30 (11.86) & 9.39 (11.45) & 0.003\\
Pack Years & 53.05 (26.63) & 47.57 (24.99) & $<$0.001\\
Airway Wall Thickness & 1.17 (0.23) & 1.00 (0.21) & $<$0.001\\
Non-Hispanic White (\%) & 82 & 78 & 0.084\\
Current Smoker (\%) & 66 & 65 & 0.510\\
Diabetes (\%) & 17 & 14 & 0.204\\
\bottomrule
\end{tabular*}
\footnotetext[]{COPD = Chronic Obstructive Pulmonary Disease}
\footnotetext[]{BMI = Body Mass Index}
\footnotetext[]{FEV$_1$ = Forced Expiratory Volume in 1 Second}
\footnotetext[]{BODE = \underline{B}ody mass index, airflow \underline{O}bstruction, \underline{D}yspnea, and \underline{E}xercise capacity}
\end{table}

==> Tables/Tab_RDA_grid_v_rand.tex <==
% Last updated 07MAY2023

\begin{table}[htbp]
\caption{Variables Selected by Random and Grid Searches Using HIP. There is strong agreement in the variables selected using either search method.}\label{tab_RDA_grid_v_rand}%
\begin{tabular}{@{}ccccc@{}}
\toprule
Data & Subtype & Random & Grid & Overlap between Random and Grid\\
\midrule
 & Males & 50 & 50 & 50\\
\cmidrule{2-5}
 & Females & 50 & 50 & 48\\
\cmidrule{2-5}
\multirow[t]{-3}{*}{\centering\arraybackslash Genes} & Common & 46 & 47 & 45\\
\cmidrule{1-5}
 & Males & 22 & 20 & 20\\
\cmidrule{2-5}
 & Females & 20 & 20 & 20\\
\cmidrule{2-5}
\multirow[t]{-3}{*}{\centering\arraybackslash Proteins} & Common & 9 & 8 & 8\\
\bottomrule
\end{tabular}
\end{table}

==> Tables/Tab_RDA_pathways.tex <==
% Last updated 09MAY2023

\begin{sidewaystable}[htbp]
\caption{Top Canonical Pathways from IPA Enrichment Analysis}\label{tab_RDA_pathways}%
%
\begin{tabular*}{\textwidth}{@{\extracolsep\fill}p{0.25cm}p{0.25cm}p{8cm}p{3.5cm}p{1.25cm}}
\toprule
View & Subgroup &	Canonical Pathway	&	Molecules	&	Unadjusted P-value\\
\midrule
\multirow{20}{*}{\centering Genes}	&	\multirow{10}{*}{\centering Males}	&	Iron homeostasis signaling pathway	&	CDC34,FECH,SLC25A37	&	0.003	\\
	&		&	Methylglyoxal Degradation I	&	HAGH	&	0.006	\\
	&		&	Heme Biosynthesis from Uroporphyrinogen-III I	&	FECH	&	0.008	\\
	&		&	Pentose Phosphate Pathway (Non-oxidative Branch)	&	RPIA	&	0.013	\\
	&		&	Heme Biosynthesis II	&	FECH	&	0.019	\\
	&		&	Pentose Phosphate Pathway	&	RPIA	&	0.023	\\
	&		&	Erythropoietin Signaling Pathway	&	BCL2L1,GATA1	&	0.054	\\
	&		&	ID1 Signaling Pathway	&	BCL2L1,GSPT1	&	0.068	\\
	&		&	Sertoli Cell-Sertoli Cell Junction Signaling	&	SPTB,YBX3	&	0.069	\\
	&		&	Autophagy	&	GABARAPL2,SLC1A5	&	0.076	\\
									
    \cmidrule(lr){2-5}
         
&	\multirow{10}{*}{\centering Females}	&	Heme Biosynthesis II	&	ALAS2,FECH	&	$<$0.001	\\
&		&	Iron homeostasis signaling pathway	&	ALAS2,CDC34,FECH,SLC25A37	&	$<$0.001	\\
&		&	Methylglyoxal Degradation I	&	HAGH	&	0.006	\\
&		&	Heme Biosynthesis from Uroporphyrinogen-III I	&	FECH	&	0.008	\\
&		&	Tetrapyrrole Biosynthesis II	&	ALAS2	&	0.010	\\
&		&	Hypoxia Signaling in the Cardiovascular System	&	CDC34,UBE2H	&	0.011	\\
&		&	Pentose Phosphate Pathway (Non-oxidative Branch)	&	RPIA	&	0.013	\\
&		&	Pentose Phosphate Pathway	&	RPIA	&	0.023	\\
&		&	Erythropoietin Signaling Pathway	&	BCL2L1,GATA1	&	0.054	\\
&		&	ID1 Signaling Pathway	&	BCL2L1,GSPT1	&	0.068	\\

 \midrule 
									
\multirow{20}{*}{\centering Proteins}	&	\multirow{10}{*}{\centering Males}	&	Role of JAK2 in Hormone-like Cytokine Signaling	&	EPO,LEP,PTPN6	&	$<$0.001	\\
	&		&	White Adipose Tissue Browning Pathway	&	BDNF,LEP,NPPB	&	$<$0.001	\\
	&		&	Erythropoietin Signaling Pathway	&	EPO,LEP,PTPN6	&	$<$0.001	\\
	&		&	Serotonin Receptor Signaling	&	ADIPOQ,BDNF,LEP,NPPB	&	$<$0.001	\\
	&		&	AMPK Signaling	&	ADIPOQ,INS,LEP	&	0.001	\\
	&		&	Leptin Signaling in Obesity	&	INS,LEP	&	0.002	\\
	&		&	IL-3 Signaling	&	PPP3R1,PTPN6	&	0.002	\\
	&		&	Maturity Onset Diabetes of Young (MODY) Signaling	&	ADIPOQ,INS	&	0.002	\\
	&		&	Thyroid Cancer Signaling	&	BDNF,INS	&	0.002	\\
	&		&	ABRA Signaling Pathway	&	NPPB,PPP3R1	&	0.003	\\

   \cmidrule(lr){2-5}
									
	&	\multirow{10}{*}{\centering Females}	&	Granulocyte Adhesion and Diapedesis	&	PF4,PPBP,TNFRSF1A	&	$<$0.001	\\
	&		&	Agranulocyte Adhesion and Diapedesis	&	PF4,PPBP,TNFRSF1A	&	$<$0.001	\\
	&		&	Wound Healing Signaling Pathway	&	EGF,PF4,TNFRSF1A	&	$<$0.001	\\
	&		&	Huntington's Disease Signaling	&	BDNF,CPLX2,EGF	&	0.001	\\
	&		&	Pathogen Induced Cytokine Storm Signaling Pathway	&	PF4,PPBP,TNFRSF1A	&	0.002	\\
	&		&	Glioma Signaling	&	CDKN2D,EGF	&	0.004	\\
	&		&	Type II Diabetes Mellitus Signaling	&	ADIPOQ,TNFRSF1A	&	0.005	\\
	&		&	Axonal Guidance Signaling	&	BDNF,EGF,PAPPA	&	0.005	\\
	&		&	Tumor Microenvironment Pathway	&	EGF,TNFRSF1A	&	0.007	\\
	&		&	Regulation Of The Epithelial Mesenchymal Transition By Growth Factors Pathway	&	EGF,TNFRSF1A	&	0.008	\\
\bottomrule
\end{tabular*}
\end{sidewaystable}

==> Tables/Tab_RDA_reg.tex <==
% Last updated on 05MAY2023
% When update, ensure to fix $<$

% 01JUN2023: Update "Gender" to "Sex"

\begin{table}[htbp]
\caption{Comparison of Regression Model Estimates. Models were fit on all participants in the COPD Data set with age, BMI, race, and pack years ($N=1374$). Scores were developed using the variables selected by HIP (Random).}\label{tab_RDA_reg}%
\begin{tabular}{@{}cccccc@{}}
%p{5cm}p{1cm}p{2cm}p{1cm}p{1cm}p{1cm}
\toprule
\Centering{Variable} & Estimate & \Centering{95\% CI} & P-value & $R^2$ & Adjusted $R^2$\\
\midrule
\multicolumn{1}{l}{\textbf{ERF}} &  &  &  & 0.112 & 0.109\\
Intercept & -0.008 & -0.078,  0.063 & 0.828 &  & \\
Age & -0.068 & -0.120, -0.015 & 0.012 &  & \\
Sex (Female vs Male) & -0.002 & -0.103,  0.099 & 0.974 &  & \\
Race (African American vs White) & 0.043 & -0.089,  0.175 & 0.525 &  & \\
BMI & 0.308 & 0.258,  0.358 & $<$0.001 &  & \\
Pack Years & 0.098 & 0.047,  0.148 & $<$0.001 &  & \\
\multicolumn{1}{l}{\textbf{ERF + Common Protein Score}} &  &  &  & 0.118 & 0.114\\
Intercept & -0.013 & -0.083,  0.058 & 0.727 &  & \\
Age & -0.056 & -0.109, -0.003 & 0.040 &  & \\
Sex (Female vs Male) & -0.003 & -0.103,  0.098 & 0.959 &  & \\
Race (African American vs White) & 0.069 & -0.064,  0.202 & 0.311 &  & \\
BMI & 0.278 & 0.225,  0.331 & $<$0.001 &  & \\
Pack Years & 0.100 & 0.049,  0.150 & $<$0.001 &  & \\
Common Protein Score & 0.087 & 0.034,  0.141 & 0.001 &  & \\
\multicolumn{1}{l}{\textbf{ERF + Common Gene Score}} &  &  &  & 0.112 & 0.108\\
Intercept & -0.007 & -0.078,  0.063 & 0.843 &  & \\
Age & -0.068 & -0.121, -0.015 & 0.012 &  & \\
Sex (Female vs Male) & -0.002 & -0.102,  0.099 & 0.977 &  & \\
Race (African American vs White) & 0.039 & -0.094,  0.173 & 0.566 &  & \\
BMI & 0.305 & 0.253,  0.357 & $<$0.001 &  & \\
Pack Years & 0.098 & 0.047,  0.148 & $<$0.001 &  & \\
Common Gene Score & 0.011 & -0.041,  0.064 & 0.672 &  & \\
\multicolumn{1}{l}{\textbf{ERF + Common Scores}} &  &  &  & 0.118 & 0.114\\
Intercept & -0.012 & -0.082,  0.058 & 0.737 &  & \\
Age & -0.056 & -0.109, -0.003 & 0.039 &  & \\
Sex (Female vs Male) & -0.003 & -0.103,  0.098 & 0.960 &  & \\
Race (African American vs White) & 0.066 & -0.068,  0.200 & 0.334 &  & \\
BMI & 0.276 & 0.221,  0.331 & $<$0.001 &  & \\
Pack Years & 0.100 & 0.049,  0.150 & $<$0.001 &  & \\
Common Protein Score & 0.087 & 0.033,  0.141 & 0.002 &  & \\
Common Gene Score & 0.007 & -0.045,  0.060 & 0.782 &  & \\
\multicolumn{1}{l}{\textbf{ERF + Subgroup Protein Score}} &  &  &  & 0.128 & 0.124\\
Intercept & -0.015 & -0.085,  0.054 & 0.665 &  & \\
Age & -0.077 & -0.129, -0.025 & 0.004 &  & \\
Sex (Female vs Male) & -0.003 & -0.103,  0.097 & 0.949 &  & \\
Race (African American vs White) & 0.085 & -0.047,  0.217 & 0.209 &  & \\
BMI & 0.263 & 0.210,  0.316 & $<$0.001 &  & \\
Pack Years & 0.099 & 0.049,  0.150 & $<$0.001 &  & \\
Subgroup Protein Score & 0.136 & 0.083,  0.190 & $<$0.001 &  & \\
\multicolumn{1}{l}{\textbf{ERF + Subgroup Gene Score}} &  &  &  & 0.112 & 0.108\\
Intercept & -0.007 & -0.078,  0.063 & 0.844 &  & \\
Age & -0.068 & -0.121, -0.015 & 0.012 &  & \\
Sex (Female vs Male) & -0.002 & -0.102,  0.099 & 0.977 &  & \\
Race (African American vs White) & 0.039 & -0.095,  0.173 & 0.567 &  & \\
BMI & 0.305 & 0.253,  0.357 & $<$0.001 &  & \\
Pack Years & 0.098 & 0.047,  0.148 & $<$0.001 &  & \\
Subgroup Gene Score & 0.011 & -0.041,  0.064 & 0.669 &  & \\
\multicolumn{1}{l}{\textbf{ERF + Subgroup Scores}} &  &  &  & 0.128 & 0.123\\
Intercept & -0.015 & -0.085,  0.055 & 0.670 &  & \\
Age & -0.077 & -0.130, -0.025 & 0.004 &  & \\
Sex (Female vs Male) & -0.003 & -0.103,  0.097 & 0.950 &  & \\
Race (African American vs White) & 0.084 & -0.050,  0.217 & 0.220 &  & \\
BMI & 0.262 & 0.208,  0.316 & $<$0.001 &  & \\
Pack Years & 0.099 & 0.049,  0.150 & $<$0.001 &  & \\
Subgroup Protein Score & 0.136 & 0.083,  0.190 & $<$0.001 &  & \\
Subtype Gene Score & 0.003 & -0.049,  0.055 & 0.897 &  & \\
\bottomrule
\multicolumn{6}{l}{\textsuperscript{} ERF = Established Risk Factors (Age, BMI, Sex, Race, and Pack Years)}\\
\multicolumn{6}{l}{\textsuperscript{} BMI = Body Mass Index}\\
\end{tabular}
\end{table}

==> Tables/Tab_RDA_regv2.tex <==
% last updated 04JUN2023

% manual updates: escape "%", add "$" around "<"

%\begin{longtable}{p{4cm}p{1.25cm}p{2.25cm}p{1.25cm}p{1.25cm}p{1.25cm}}
%\caption{V2}
%\label{tab:regv2}\\

\renewcommand{\arraystretch}{0.5}

\begin{table}[htbp]
\caption{Comparison of Regression Model Estimates. Models were fit on all participants in the COPD Data set and adjusted for age, sex, race, BMI, smoking status, percent emphysema, and scanner make ($N=1374$). Scores were developed using the stable proteins and genes selected by HIP (Random).}\label{tab_RDA_reg}%
\begin{tabular*}{\textwidth}{@{\extracolsep\fill}cccccc}
\toprule
Variable & Estimate & 95\% CI & P-value & $R^2$ & Adjusted $R^2$\\
\midrule
\multicolumn{1}{l}{\textbf{ERF}} &  &  &  & 0.152 & 0.147\\
Intercept & -1.180 & -1.872, -0.489 & 0.001 &  & \\
Age & 0.021 & -0.035,  0.077 & 0.461 &  & \\
Sex (Female) & 0.006 & -0.093,  0.105 & 0.901 &  & \\
Race (African American) & -0.070 & -0.202,  0.062 & 0.297 &  & \\
BMI & 0.352 & 0.299,  0.406 & $<$0.001 &  & \\
Former Smoker & 0.947 & 0.257,  1.637 & 0.007 &  & \\
Current Smoker & 1.429 & 0.735,  2.123 & $<$0.001 &  & \\
\% Emphysema & 0.023 & -0.032,  0.079 & 0.414 &  & \\
Scanner - Philips & 0.379 & 0.097,  0.661 & 0.009 &  & \\
Scanner - Siemens & 0.130 & 0.025,  0.235 & 0.015 &  & \\
\multicolumn{1}{l}{\textbf{ERF + Common Protein Score}} &  &  &  & 0.157 & 0.151\\
Intercept & -1.138 & -1.828, -0.447 & 0.001 &  & \\
Age & 0.032 & -0.024,  0.089 & 0.266 &  & \\
Sex (Female) & 0.007 & -0.092,  0.105 & 0.897 &  & \\
Race (African American) & -0.049 & -0.181,  0.084 & 0.469 &  & \\
BMI & 0.327 & 0.271,  0.383 & $<$0.001 &  & \\
Former Smoker & 0.911 & 0.223,  1.600 & 0.010 &  & \\
Current Smoker & 1.390 & 0.697,  2.083 & $<$0.001 &  & \\
\% Emphysema & 0.028 & -0.028,  0.083 & 0.328 &  & \\
Scanner - Philips & 0.404 & 0.123,  0.686 & 0.005 &  & \\
Scanner - Siemens & 0.110 & 0.005,  0.216 & 0.041 &  & \\
Common Protein Score & 0.076 & 0.023,  0.130 & 0.005 &  & \\
\multicolumn{1}{l}{\textbf{ERF + Common Gene Score}} &  &  &  & 0.153 & 0.147\\
Intercept & -1.169 & -1.861, -0.477 & 0.001 &  & \\
Age & 0.021 & -0.035,  0.077 & 0.462 &  & \\
Sex (Female) & 0.007 & -0.092,  0.106 & 0.893 &  & \\
Race (African American) & -0.083 & -0.216,  0.050 & 0.221 &  & \\
BMI & 0.343 & 0.288,  0.398 & $<$0.001 &  & \\
Former Smoker & 0.932 & 0.242,  1.623 & 0.008 &  & \\
Current Smoker & 1.423 & 0.729,  2.117 & $<$0.001 &  & \\
\% Emphysema & 0.023 & -0.033,  0.079 & 0.421 &  & \\
Scanner - Philips & 0.387 & 0.105,  0.669 & 0.007 &  & \\
Scanner - Siemens & 0.134 & 0.029,  0.239 & 0.013 &  & \\
Common Gene Score & 0.035 & -0.017,  0.086 & 0.185 &  & \\
\multicolumn{1}{l}{\textbf{ERF + Common Scores}} &  &  &  & 0.158 & 0.151\\
Intercept & -1.128 & -1.819, -0.437 & 0.001 &  & \\
Age & 0.032 & -0.025,  0.088 & 0.270 &  & \\
Sex (Female) & 0.007 & -0.092,  0.106 & 0.890 &  & \\
Race (African American) & -0.061 & -0.195,  0.073 & 0.373 &  & \\
BMI & 0.320 & 0.262,  0.377 & $<$0.001 &  & \\
Former Smoker & 0.899 & 0.210,  1.588 & 0.011 &  & \\
Current Smoker & 1.385 & 0.692,  2.078 & $<$0.001 &  & \\
\% Emphysema & 0.027 & -0.028,  0.083 & 0.335 &  & \\
Scanner - Philips & 0.411 & 0.129,  0.693 & 0.004 &  & \\
Scanner - Siemens & 0.114 & 0.008,  0.220 & 0.035 &  & \\
Common Protein Score & 0.074 & 0.021,  0.128 & 0.006 &  & \\
Common Gene Score & 0.031 & -0.020,  0.083 & 0.237 &  & \\
\multicolumn{1}{l}{\textbf{ERF + Subgroup Protein Score}} &  &  &  & 0.165 & 0.159\\
Intercept & -1.071 & -1.760, -0.383 & 0.002 &  & \\
Age & 0.014 & -0.041,  0.070 & 0.614 &  & \\
Sex (Female) & 0.007 & -0.091,  0.105 & 0.891 &  & \\
Race (African American) & -0.035 & -0.167,  0.097 & 0.605 &  & \\
BMI & 0.312 & 0.256,  0.368 & $<$0.001 &  & \\
Former Smoker & 0.860 & 0.174,  1.546 & 0.014 &  & \\
Current Smoker & 1.335 & 0.645,  2.025 & $<$0.001 &  & \\
\% Emphysema & 0.030 & -0.025,  0.086 & 0.284 &  & \\
Scanner - Philips & 0.418 & 0.137,  0.698 & 0.004 &  & \\
Scanner - Siemens & 0.079 & -0.027,  0.185 & 0.146 &  & \\
Subgroup Protein Score & 0.126 & 0.072,  0.179 & $<$0.001 &  & \\
\multicolumn{1}{l}{\textbf{ERF + Subgroup Gene Score}} &  &  &  & 0.153 & 0.147\\
Intercept & -1.169 & -1.861, -0.477 & 0.001 &  & \\
Age & 0.021 & -0.035,  0.077 & 0.459 &  & \\
Sex (Female) & 0.007 & -0.092,  0.106 & 0.893 &  & \\
Race (African American) & -0.083 & -0.217,  0.050 & 0.220 &  & \\
BMI & 0.343 & 0.288,  0.398 & $<$0.001 &  & \\
Former Smoker & 0.932 & 0.242,  1.622 & 0.008 &  & \\
Current Smoker & 1.423 & 0.729,  2.117 & $<$0.001 &  & \\
\% Emphysema & 0.023 & -0.033,  0.079 & 0.421 &  & \\
Scanner - Philips & 0.387 & 0.105,  0.669 & 0.007 &  & \\
Scanner - Siemens & 0.134 & 0.029,  0.239 & 0.013 &  & \\
Subgroup Gene Score & 0.035 & -0.016,  0.087 & 0.180 &  & \\
\multicolumn{1}{l}{\textbf{ERF + Subgroup Scores}} &  &  &  & 0.166 & 0.159\\
Intercept & -1.064 & -1.752, -0.375 & 0.003 &  & \\
Age & 0.015 & -0.041,  0.070 & 0.610 &  & \\
Sex (Female) & 0.007 & -0.091,  0.106 & 0.885 &  & \\
Race (African American) & -0.045 & -0.179,  0.088 & 0.504 &  & \\
BMI & 0.306 & 0.249,  0.363 & $<$0.001 &  & \\
Former Smoker & 0.850 & 0.164,  1.536 & 0.015 &  & \\
Current Smoker & 1.332 & 0.642,  2.022 & $<$0.001 &  & \\
\% Emphysema & 0.030 & -0.025,  0.085 & 0.290 &  & \\
Scanner - Philips & 0.423 & 0.142,  0.704 & 0.003 &  & \\
Scanner - Siemens & 0.083 & -0.024,  0.189 & 0.129 &  & \\
Subgroup Protein Score & 0.124 & 0.070,  0.177 & $<$0.001 &  & \\
Subtype Gene Score & 0.027 & -0.024,  0.078 & 0.304 &  & \\
\bottomrule
\end{tabular*}
\footnotetext[]{ERF = Established Risk Factors (Age, Sex, Race, BMI, and Smoking Status)}
\footnotetext[]{BMI = Body Mass Index}
\end{table}

==> Tables/Tab_RDA_scores.tex <==
% Last updated on 05MAY2023


\begin{sidewaystable}[htbp]
\caption{Average Train and Test MSEs. The data was split 100 times into a test and training set. Scores were developed using the variables selected by HIP (Random).}\label{tab_RDA_scores}%
\begin{tabular*}{\textheight}{@{\extracolsep\fill}lccccclcc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Train MSE} & \multicolumn{3}{c}{Test MSE} & \multicolumn{2}{c}{ } \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){5-7}
Model & Overall & Males & Females & Overall & Males & Females & $R^2$ & Adjusted $R^2$\\
\midrule
ERF & 0.889 & 0.903 & 0.871 & 0.890 & 0.900 & 0.877 & 0.115 & 0.110\\
ERF + Common Protein Score & 0.883 & 0.901 & 0.859 & 0.885 & 0.899 & 0.866 & 0.122 & 0.115\\
ERF + Common Gene Score & 0.889 & 0.903 & 0.870 & 0.892 & 0.902 & 0.878 & 0.116 & 0.109\\
ERF + Common Scores & 0.882 & 0.900 & 0.859 & 0.887 & 0.901 & 0.868 & 0.122 & 0.115\\
ERF + Subtype Protein Score & 0.873 & 0.888 & 0.853 & 0.875 & 0.887 & 0.860 & 0.132 & 0.125\\
ERF + Subtype Gene Score & 0.889 & 0.903 & 0.870 & 0.892 & 0.902 & 0.878 & 0.116 & 0.109\\
ERF + Subtype Scores & 0.873 & 0.888 & 0.853 & 0.877 & 0.889 & 0.862 & 0.132 & 0.125\\
ERF + Opposite Subtype Protein Score & 0.881 & 0.896 & 0.862 & 0.884 & 0.894 & 0.870 & 0.123 & 0.117\\
ERF + Opposite Subtype Gene Score & 0.889 & 0.903 & 0.870 & 0.892 & 0.902 & 0.878 & 0.116 & 0.109\\
ERF + Opposite Subtype Scores & 0.881 & 0.896 & 0.862 & 0.885 & 0.896 & 0.872 & 0.124 & 0.116\\
\bottomrule
\multicolumn{9}{l}{\textsuperscript{} ERF = Established Risk Factors (Age, BMI, Sex, Race, and Pack Years)}\\
\end{tabular*}
\end{sidewaystable}

==> Tables/Tab_RDA_scoresv2.tex <==
% last updated 04JUN2023

% manual updates:

\begin{sidewaystable}[htbp]
\caption{Average Train and Test MSEs. The data was split 100 times into a test and training set. Scores were developed using the variables selected by HIP (Random).}\label{tab_RDA_scoresv2}%
\begin{tabular}{lccccclcc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Train MSE} & \multicolumn{3}{c}{Test MSE} & \multicolumn{2}{c}{ } \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){5-7}
Model & Overall & Males & Females & Overall & Males & Females & $R^2$ & Adjusted $R^2$\\
\midrule
ERF & 0.848 & 0.858 & 0.834 & 0.855 & 0.863 & 0.844 & 0.156 & 0.147\\
ERF + Common Protein Score & 0.843 & 0.858 & 0.823 & 0.851 & 0.864 & 0.834 & 0.161 & 0.151\\
ERF + Common Gene Score & 0.847 & 0.857 & 0.832 & 0.855 & 0.864 & 0.844 & 0.158 & 0.148\\
ERF + Common Scores & 0.842 & 0.857 & 0.822 & 0.852 & 0.865 & 0.835 & 0.163 & 0.151\\
ERF + Subtype Protein Score & 0.835 & 0.848 & 0.818 & 0.843 & 0.854 & 0.829 & 0.170 & 0.159\\
ERF + Subtype Gene Score & 0.847 & 0.857 & 0.833 & 0.855 & 0.864 & 0.844 & 0.158 & 0.148\\
ERF + Subtype Scores & 0.834 & 0.847 & 0.817 & 0.844 & 0.855 & 0.830 & 0.170 & 0.159\\
ERF + Opposite Subtype Protein Score & 0.843 & 0.855 & 0.826 & 0.851 & 0.861 & 0.838 & 0.162 & 0.151\\
ERF + Opposite Subtype Gene Score & 0.847 & 0.857 & 0.833 & 0.855 & 0.864 & 0.844 & 0.158 & 0.147\\
ERF + Opposite Subtype Scores & 0.841 & 0.854 & 0.824 & 0.852 & 0.862 & 0.838 & 0.163 & 0.152\\
\bottomrule
\multicolumn{9}{l}{\textsuperscript{} ERF = Established Risk Factors (Age, Sex, Race, BMI, and Smoking Status)}\\
\end{tabular}
\end{sidewaystable}

==> Tables/Tab_RDA_split_selected.tex <==
% Last uppdated 12MAY2023

\begin{table}[htbp]
\caption{Number of variables selected by each method from 50 data splits. Values are Mean (SD).}\label{tab_RDA_split_selected}%
\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{Genes} & \multicolumn{2}{c}{Proteins} \\
\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5}
Method & Males & Females & Males & Females\\
\midrule
CVR & 260.6 (39) & 194.9 (72) & 153 (26.3) & 153 (26.3)\\
Elastic Net & 175.9 (28) & 107.8 (34.8) & 66 (9.4) & 66 (9.4)\\
HIP (Grid) & 75 (0) & 75 (0) & 25 (0) & 25 (0)\\
HIP (Random) & 75 (0) & 75 (0) & 25 (0) & 25 (0)\\
Joint Lasso & 781.1 (62.8) & 777.3 (61.8) & 256.5 (81.5) & 256.5 (81.5)\\
Lasso & 167.9 (28.3) & 94.3 (36.2) & 62.8 (8.5) & 62.8 (8.5)\\
\bottomrule
\end{tabular}
\end{table}

==> Tables/Tab_RDA_top_vars.tex <==
% Last updated 02MAY2023

\begin{table}[htbp]
\caption{Number of Variables Selected by Each Method. The top 1\% (of the 5000 genes and 2000 proteins retained from unsupervised filtering) most frequently selected genes and proteins across 50 random splits of the data are considered 'selected'.}\label{tab_RDA_top_vars}%
\begin{tabular}{@{}lcccccc@{}}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Genes} & \multicolumn{3}{c}{Proteins} \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){5-7}
Method & Males & Females & Common & Males & Females & Common\\
\midrule
HIP (Random) & 50 & 50 & 46 & 22 & 20 & 9\\
HIP (Grid) & 50 & 50 & 47 & 20 & 20 & 8\\
Joint Lasso & 64 & 63 & 48 & 34 & 38 & 29\\
CVR & 50 & 50 & 15 & 21 & 23 & 12\\
Lasso & 50 & 50 & 4 & 20 & 20 & 5\\
Elastic Net & 52 & 50 & 6 & 20 & 20 & 6\\
\bottomrule
\end{tabular}
\end{table}

==> Tables/Tab_RDA_weights_gene_F.tex <==
% Last updated 09MAY2023

%begin{tabular*}{\textwidth}{@{\extracolsep\fill}lcccccc}
%\toprule%
%& \multicolumn{3}{@{}c@{}}{Element 1\footnotemark[1]} & \multicolumn{3}{@{}c@{}}{Element 2\footnotemark[2]} \\\cmidrule{2-4}\cmidrule{5-7}%

\begin{table}[htbp]
\caption{List of Genes Selected by HIP (Random) for Females in COPD Application. Weights are an average calculated from the estimated $\bm B^{d,s}$ matrices. Higher values suggest the variable likely contributes more to association and prediction.}\label{tab_RDA_weights_geneF}%
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}p{1in}p{2in}p{0.5in}p{0.5in}}
\toprule%
ID & Name & Symbol & Weight\\
\midrule
ENSG00000171552.14 & BCL2 like 1 & BCL2L1 & 1.162\\
ENSG00000159346.13 & adiponectin receptor 1 & ADIPOR1 & 1.155\\
ENSG00000198876.13 & DDB1 and CUL4 associated factor 12 & DCAF12 & 1.152\\
ENSG00000130821.17 & solute carrier family 6 member 8 & SLC6A8 & 1.145\\
ENSG00000124098.10 & family with sequence similarity 210 member B & FAM210B & 1.140\\
ENSG00000130830.15 & MAGUK p55 scaffold protein 1 & MPP1 & 1.135\\
ENSG00000137198.10 & guanosine monophosphate reductase & GMPR & 1.129\\
ENSG00000073792.16 & insulin like growth factor 2 mRNA binding protein 2 & IGF2BP2 & 1.128\\
ENSG00000082146.13 & STE20 related adaptor beta & STRADB & 1.127\\
ENSG00000060138.13 & Y-box binding protein 3 & YBX3 & 1.127\\
ENSG00000166947.15 & erythrocyte membrane protein band 4.2 & EPB42 & 1.125\\
ENSG00000133606.11 & makorin ring finger protein 1 & MKRN1 & 1.125\\
ENSG00000119950.21 & MAX interactor 1, dimerization protein & MXI1 & 1.122\\
ENSG00000158856.18 & dematin actin binding protein & DMTN & 1.122\\
ENSG00000168785.8 & tetraspanin 5 & TSPAN5 & 1.120\\
ENSG00000143416.21 & selenium binding protein 1 & SELENBP1 & 1.119\\
ENSG00000066926.12 & ferrochelatase & FECH & 1.117\\
ENSG00000183508.5 & terminal nucleotidyltransferase 5C & TENT5C & 1.116\\
ENSG00000013306.16 & solute carrier family 25 member 39 & SLC25A39 & 1.116\\
ENSG00000133193.12 & family with sequence similarity 104 member A & FAM104A & 1.115\\
ENSG00000099804.9 & cell division cycle 34, ubiqiutin conjugating enzyme & CDC34 & 1.114\\
ENSG00000162722.9 & tripartite motif containing 58 & TRIM58 & 1.113\\
ENSG00000105701.16 & FKBP prolyl isomerase 8 & FKBP8 & 1.111\\
ENSG00000022840.16 & ring finger protein 10 & RNF10 & 1.111\\
ENSG00000143321.19 & heparin binding growth factor & HDGF & 1.110\\
ENSG00000182512.5 & glutaredoxin 5 & GLRX5 & 1.110\\
ENSG00000167671.12 & UBX domain protein 6 & UBXN6 & 1.110\\
ENSG00000196961.13 & adaptor related protein complex 2 subunit alpha 1 & AP2A1 & 1.108\\
ENSG00000147454.14 & solute carrier family 25 member 37 & SLC25A37 & 1.108\\
ENSG00000070182.21 & spectrin beta, erythrocytic & SPTB & 1.108\\
ENSG00000004939.15 & solute carrier family 4 member 1 (Diego blood group) & SLC4A1 & 1.107\\
ENSG00000102145.15 & GATA binding protein 1 & GATA1 & 1.103\\
ENSG00000103342.13 & G1 to S phase transition 1 & GSPT1 & 1.101\\
ENSG00000079308.19 & tensin 1 & TNS1 & 1.101\\
ENSG00000132819.17 & RNA binding motif protein 38 & RBM38 & 1.100\\
ENSG00000100614.18 & protein phosphatase, Mg2+/Mn2+ dependent 1A & PPM1A & 1.098\\
ENSG00000101782.15 & RIO kinase 3 & RIOK3 & 1.095\\
ENSG00000137216.19 & transmembrane protein 63B & TMEM63B & 1.090\\
ENSG00000167705.12 & Rab interacting lysosomal protein & RILP & 1.086\\
ENSG00000063854.13 & hydroxyacylglutathione hydrolase & HAGH & 1.081\\
ENSG00000143774.17 & guanylate kinase 1 & GUK1 & 1.075\\
ENSG00000047597.7 & X-linked Kx blood group antigen, Kell and VPS13A binding protein & XK & 1.073\\
ENSG00000129472.15 & RAB2B, member RAS oncogene family & RAB2B & 1.072\\
ENSG00000186591.13 & ubiquitin conjugating enzyme E2 H & UBE2H & 1.070\\
ENSG00000153574.9 & ribose 5-phosphate isomerase A & RPIA & 1.069\\
ENSG00000105281.12 & solute carrier family 1 member 5 & SLC1A5 & 1.066\\
ENSG00000162367.11 & TAL bHLH transcription factor 1, erythroid differentiation factor & TAL1 & 1.064\\
ENSG00000181788.4 & siah E3 ubiquitin protein ligase 2 & SIAH2 & 1.064\\
ENSG00000158578.21 & 5'-aminolevulinate synthase 2 & ALAS2 & 1.040\\
ENSG00000204613.11 & tripartite motif containing 10 & TRIM10 & 1.039\\
\bottomrule
\end{tabular*}
\end{table}

==> Tables/Tab_RDA_weights_gene_M.tex <==
% Last updated 09MAY2023

\begin{table}[htbp]
\caption{List of Genes Selected by HIP (Random) for Males in COPD Application. Weights are an average calculated from the estimated $\bm B^{d,s}$ matrices. Higher values suggest the variable likely contributes more to association and prediction.}\label{tab_RDA_weights_geneM}%
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}p{1in}p{2in}p{0.5in}p{0.5in}}
\toprule
ID & Name & Symbol & Weight\\
\midrule
ENSG00000159346.13 & adiponectin receptor 1 & ADIPOR1 & 1.121\\
ENSG00000124098.10 & family with sequence similarity 210 member B & FAM210B & 1.112\\
ENSG00000130830.15 & MAGUK p55 scaffold protein 1 & MPP1 & 1.107\\
ENSG00000198876.13 & DDB1 and CUL4 associated factor 12 & DCAF12 & 1.102\\
ENSG00000099804.9 & cell division cycle 34, ubiqiutin conjugating enzyme & CDC34 & 1.101\\
ENSG00000137198.10 & guanosine monophosphate reductase & GMPR & 1.100\\
ENSG00000133193.12 & family with sequence similarity 104 member A & FAM104A & 1.100\\
ENSG00000171552.14 & BCL2 like 1 & BCL2L1 & 1.098\\
ENSG00000147454.14 & solute carrier family 25 member 37 & SLC25A37 & 1.097\\
ENSG00000167671.12 & UBX domain protein 6 & UBXN6 & 1.096\\
ENSG00000119950.21 & MAX interactor 1, dimerization protein & MXI1 & 1.095\\
ENSG00000196961.13 & adaptor related protein complex 2 subunit alpha 1 & AP2A1 & 1.093\\
ENSG00000143321.19 & heparin binding growth factor & HDGF & 1.092\\
ENSG00000168785.8 & tetraspanin 5 & TSPAN5 & 1.091\\
ENSG00000166947.15 & erythrocyte membrane protein band 4.2 & EPB42 & 1.089\\
ENSG00000143416.21 & selenium binding protein 1 & SELENBP1 & 1.088\\
ENSG00000022840.16 & ring finger protein 10 & RNF10 & 1.085\\
ENSG00000101782.15 & RIO kinase 3 & RIOK3 & 1.085\\
ENSG00000158856.18 & dematin actin binding protein & DMTN & 1.085\\
ENSG00000105701.16 & FKBP prolyl isomerase 8 & FKBP8 & 1.085\\
ENSG00000133606.11 & makorin ring finger protein 1 & MKRN1 & 1.084\\
ENSG00000066926.12 & ferrochelatase & FECH & 1.084\\
ENSG00000183508.5 & terminal nucleotidyltransferase 5C & TENT5C & 1.081\\
ENSG00000100614.18 & protein phosphatase, Mg2+/Mn2+ dependent 1A & PPM1A & 1.081\\
ENSG00000182512.5 & glutaredoxin 5 & GLRX5 & 1.079\\
ENSG00000079308.19 & tensin 1 & TNS1 & 1.077\\
ENSG00000070182.21 & spectrin beta, erythrocytic & SPTB & 1.077\\
ENSG00000013306.16 & solute carrier family 25 member 39 & SLC25A39 & 1.074\\
ENSG00000162722.9 & tripartite motif containing 58 & TRIM58 & 1.074\\
ENSG00000167705.12 & Rab interacting lysosomal protein & RILP & 1.074\\
ENSG00000130821.17 & solute carrier family 6 member 8 & SLC6A8 & 1.071\\
ENSG00000103342.13 & G1 to S phase transition 1 & GSPT1 & 1.070\\
ENSG00000082146.13 & STE20 related adaptor beta & STRADB & 1.069\\
ENSG00000143774.17 & guanylate kinase 1 & GUK1 & 1.069\\
ENSG00000034713.8 & GABA type A receptor associated protein like 2 & GABARAPL2 & 1.061\\
ENSG00000102145.15 & GATA binding protein 1 & GATA1 & 1.061\\
ENSG00000063854.13 & hydroxyacylglutathione hydrolase & HAGH & 1.060\\
ENSG00000132819.17 & RNA binding motif protein 38 & RBM38 & 1.059\\
ENSG00000004939.15 & solute carrier family 4 member 1 (Diego blood group) & SLC4A1 & 1.059\\
ENSG00000060138.13 & Y-box binding protein 3 & YBX3 & 1.057\\
ENSG00000105281.12 & solute carrier family 1 member 5 & SLC1A5 & 1.055\\
ENSG00000181788.4 & siah E3 ubiquitin protein ligase 2 & SIAH2 & 1.051\\
ENSG00000136732.16 & glycophorin C (Gerbich blood group) & GYPC & 1.048\\
ENSG00000137216.19 & transmembrane protein 63B & TMEM63B & 1.047\\
ENSG00000047597.7 & X-linked Kx blood group antigen, Kell and VPS13A binding protein & XK & 1.046\\
ENSG00000153574.9 & ribose 5-phosphate isomerase A & RPIA & 1.045\\
ENSG00000100325.15 & activating signal cointegrator 1 complex subunit 2 & ASCC2 & 1.040\\
ENSG00000205639.12 & major facilitator superfamily domain containing 2B & MFSD2B & 1.040\\
ENSG00000204613.11 & tripartite motif containing 10 & TRIM10 & 1.030\\
ENSG00000129472.15 & RAB2B, member RAS oncogene family & RAB2B & 1.014\\
\bottomrule
\end{tabular*}
\end{table}

==> Tables/Tab_RDA_weights_prot.tex <==
% Last updated 07MAY2023

\begin{table}[htbp]
\caption{List of Proteins Selected by HIP (Random) in COPD Application. Weights are an average calculated from the estimated $\bm B^{d,s}$ matrices. Higher values suggest the variable likely contributes more to association and prediction.}\label{tab_RDA_weights_prot}%
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}p{0.5in}p{0.5in}p{2in}p{0.5in}p{0.5in}}
\toprule
Subgroup & ID & Name & Symbol & Weight\\
\midrule

 & 55666 & Nuclear protein localization protein 4 homolog & NPLOC4 & 1.310\\

 & 51324 & Maspardin & SPG21 & 1.273\\

 & 5196 & Platelet factor 4 & PF4 & 1.033\\

 & 2814 & Platelet glycoprotein V & GP5 & 1.032\\

 & 5473 & Beta-thromboglobulin & PPBP & 1.030\\

 & 627 & Brain-derived neurotrophic factor & BDNF & 0.962\\

 & 115761 & ADP-ribosylation factor-like protein 11 & ARL11 & 0.958\\

 & 5473 & Platelet basic protein & PPBP & 0.931\\

 & 5534 & Calcineurin subunit B type 1 & PPP3R1 & 0.925\\

 & 5777 & Tyrosine-protein phosphatase non-receptor type 6 & PTPN6 & 0.827\\

 & 10814 & Complexin-2 & CPLX2 & 0.797\\

 & 340205 & Trem-like transcript 1 protein:immunoreceptor tyrosine-based inhibition motif & TREML1 & 0.784\\

 & 81567 & Thioredoxin domain-containing protein 5 & TXNDC5 & 0.734\\

 & 4879 & N-terminal pro-BNP & NPPB & 0.729\\

 & 3485 & Insulin-like growth factor-binding protein 2 & IGFBP2 & 0.715\\

 & 2056 & Erythropoietin & EPO & 0.664\\

 & 9370 & Adiponectin & ADIPOQ & 0.586\\

 & 3630 & Insulin & INS & 0.584\\

 & 3952 & Leptin & LEP & 0.579\\

 & 5069 & Pappalysin-1 & PAPPA & 0.574\\

 & 3934 & Neutrophil gelatinase-associated lipocalin & LCN2 & 0.516\\

\multirow[t]{-22}{*}{\centering\arraybackslash Males} & 6289 & Serum amyloid A-2 protein & SAA2 & 0.446\\

\cmidrule{1-5}

 & 60682 & Stromal membrane-associated protein 1 & SMAP1 & 1.192\\

 & 1032 & Cyclin-dependent kinase 4 inhibitor D & CDKN2D & 1.188\\

 & 5473 & Connective tissue-activating peptide III & PPBP & 1.157\\

 & 2814 & Platelet glycoprotein V & GP5 & 1.156\\

 & 1950 & Epidermal growth factor:Extracellular domain & EGF & 1.133\\

 & 627 & Brain-derived neurotrophic factor & BDNF & 1.129\\

 & 5473 & Neutrophil-activating peptide 2 & PPBP & 1.116\\

 & 5196 & Platelet factor 4 & PF4 & 1.087\\

 & 5473 & Beta-thromboglobulin & PPBP & 1.072\\

 & 5473 & Platelet basic protein & PPBP & 1.068\\

 & 7132 & Tumor necrosis factor receptor superfamily member 1A & TNFRSF1A & 0.972\\

 & 10406 & WAP four-disulfide core domain protein 2 & WFDC2 & 0.921\\

 & 51087 & Y-box-binding protein 2 & YBX2 & 0.915\\

 & 4904 & Nuclease-sensitive element-binding protein 1 & YBX1 & 0.802\\

 & 10814 & Complexin-2 & CPLX2 & 0.799\\

 & 11314 & CMRF35-like molecule 8 & CD300A & 0.796\\

 & 3485 & Insulin-like growth factor-binding protein 2 & IGFBP2 & 0.700\\

 & 1088 & Carcinoembryonic antigen-related cell adhesion molecule 8 & CEACAM8 & 0.670\\

 & 5069 & Pappalysin-1 & PAPPA & 0.651\\

\multirow[t]{-20}{*}{\centering\arraybackslash Females} & 9370 & Adiponectin & ADIPOQ & 0.619\\
\bottomrule
\end{tabular*}
\end{table}
